Suboptimal Provision of Privacy and Statistical Accuracy When They are Public Goods

With vast databases at their disposal, private tech companies can compete with public statistical agencies to provide population statistics. However, private companies face different incentives to provide high-quality statistics and to protect the privacy of the people whose data are used. When both privacy protection and statistical accuracy are public goods, private providers tend to produce at least one suboptimally, but it is not clear which. We model a firm that publishes statistics under a guarantee of differential privacy. We prove that provision by the private firm results in inefficiently low data quality in this framework.

==> acknowledgements.tex <==
%TCIDATA{Version=5.50.0.2960}
%TCIDATA{LaTeXparent=0,0,sw-edit.tex}
% -*- latex -*-
%
% Time-stamp: <02/03/14 16:29:52 vilhuber>
%              Automatically adjusted if using Xemacs
%              Please adjust manually if using other editors
%
% acknowledgements.tex
% Part of abowd-schmutte-privacy.tex
Abowd and Schmutte acknowledge the support of Alfred P.\ Sloan Foundation Grant G-2015-13903 and NSF Grant SES-1131848. Abowd acknowledges direct support from the U.S.\ Census Bureau (before and during his appointment as Associate Director) and from NSF Grants BCS-0941226, TC-1012593. Some of the research for this paper was conducted using the resources of the \href{http://www2.vrdc.cornell.edu/news/social-science-gateway/}{Social Science Gateway}, which was partially supported by NSF grant SES-0922005. Any opinions and conclusions expressed herein are those of the authors and do not necessarily represent the views of the Census Bureau, NSF, or the Sloan Foundation.
%INI Requested Acknowledgement
The authors would like to thank the Isaac Newton Institute for Mathematical Sciences, Cambridge, for support and hospitality during the Programme on Data Linkage and Anonymisation, where some work on this paper was undertaken, supported by EPSRC grant no.\ EP/K032208/1.
Abowd also acknowledges the Center for Labor Economics at UC Berkeley, where he was a visiting scholar when this work was initiated.
%Helpful individual comments
We acknowledge helpful comments from Larry Blume, David Card, Michael Castro, Cynthia Dwork, John Eltinge, Stephen Fienberg, Mark Kutzbach, Ron Jarmin, Dan Kifer, Ashwin Machanavajjhala, Frank McSherry, Gerome Miklau, Kobbi Nissim, Mallesh Pai, Jerry Reiter, Eric Slud, Adam Smith, Bruce Spencer, Sara Sullivan, Lars Vilhuber and Nellie Zhao %(there must be more)
%Conferences
along with seminar and conference participants at the U.S.\ Census Bureau, Cornell University, CREST, George Mason University, Georgetown University, University of Washington Evans School of Public Policy, and the Society of Labor Economists.
We thank Jennifer Childs and Casey Eggleston for providing data from the Federal Statistical System Public Opinion Survey conducted by the Census Bureau's Center for Survey Methodology. William Sexton provided excellent research assistance.
No confidential data were used in this paper.
A complete archive of the data and programs used in this paper is available via \url{http://doi.org/10.5281/zenodo.345385}.
%%% Local Variables:
%%% mode: latex
%%% TeX-master: sw-edit
%%% End:


==> background.tex <==
%TCIDATA{Version=5.50.0.2960}
%TCIDATA{LaTeXparent=0,0,sw-edit.tex}
                      

% -*- latex -*-
%
% background.tex
% Part of abowd-schmutte-privacy.tex

\subsection{Differential Privacy and Statistical Disclosure Limitation\label%
{subsec:dpandsdl}}

% Since \citet{Fellegi:1972} and \citet{Dalenius:Towards:1977} laid out the
% problem of statistical disclosure limitation (SDL) to formalize the
% confidentiality protections that statistical agencies could provide to
% respondents, there have been many practical techniques developed and applied
% by statistical agencies and other curators of confidential data. These
% methods are nicely summarized in \citet{duncanetal2011statistical}. %
% \citet{Duncan:Risk:JBES:1986} first modeled the trade-off between the
% protection afforded by SDL and the quality/accuracy of the published
% statistics. But it is the work of Dwork and her many collaborators, see the
% bibliography in \citet{Dwork:Algorithmic:Book:2014}, in formalizing data
% privacy that has motivated much of the recent work in both computer science
% and statitical disclosure limitation, especially as it relates to mechanisms
% for buying privacy in support of privacy-preserving data analyses. The work
% of \citet{McSherry:Mechanism:FOCS07:4389483} and %
% \citet{Ghosh:2011:SPA:1993574.1993605} is most relevant to this paper.

We work with the concept of differential privacy introduced by %
\citet{dwork:2006}. To reduce confusion, we note that the SDL literature
defines confidentiality protection as the effort to ensure that a
respondent's exact identity or attributes are not disclosed in the published
data. Computer scientists define data privacy as limits on the amount of
information contained in the published data about any person in the
population, respondent or not. The two literatures have much in common but
the main point of commonality that we use here are definitions of
inferential disclosure, due to \citet{Dalenius:Towards:1977}, and
differential privacy, due to \citet{dwork:2006}.

Inferential disclosure parameterizes the confidentiality protection afforded
by a particular SDL method using the ratio of the posterior odds of
correctly assigning an identity or a sensitive attribute to a particular
respondent, given the newly released data, to the prior odds, given all
previously released data. Differential privacy parameterizes the privacy
protection in a data publishing system by bounding the same posterior odds
ratio for all potential respondents in all potential configurations of the
confidential data.


% [This paragraph needs to be revised, but is not essential for the seminar draft]

% To foreshadow what we develop below, we provide a concise summary of the
% antecedents to our work here. We adopt the differential privacy definitions
% in \citet{Blum:2008} and \citet{Hardt:Multiplicative:FOCS10} explicitly,
% noting that these are also used by \citet{Hardt:Simple:arXiv:2010}, %
% \citet{Gupta:2012:ICP:2238936.2238961} and %
% \citet{Dwork:Algorithmic:Book:2014}. Then, we consider normalized linear
% queries of the histogram representations of databases with $N$ entries. $N$
% is always the population under study, not a sample. The global sensitivity
% of all such queries is $\frac{1}{N}.$ We use the $\left( \alpha ,\beta
% \right) $-accurate query mechanism from Definition III.1 and the $\left(
% \varepsilon ,\delta \right) $-differential privacy Definition III.2 from
% Hardt and Rothblum as adapted by \citet{Gupta:2012:ICP:2238936.2238961} and %
% \citet{Dwork:Algorithmic:Book:2014}. 
% We consider only the maximally accurate
% allowable query; hence, our analysis sets their query round, $k$, at the
% allowable limit for the Private Multiplicative Weight (PWM) mechanism in
% their Figure 1, which is their parameter $c$. We implement the enhancements
% to PMW found in \citet{Gupta:2012:ICP:2238936.2238961}--in particular,
% tighter accuracy bounds and an explicit limit on the number of query rounds
% required to reach the target accuracy for given privacy loss parameters.
% Readers familiar with the data privacy literature in computer science now
% have all the necessary information to put our contribution in context. For
% the benefit of economists and statisticians, the development below is
% self-contained with a road map to relate our proofs to the relevant papers
% in the differential privacy literature.

\subsection{Statistical Data Releases and Privacy Protection Are Both Public
Goods}

Publishing statistical data, whether the output of a government agency or of
an open scientific study, involves making statistical summaries of the
information that has been collected from the population under study
available for anyone to use. Consistent with this principle, we formalize
publishing statistical data as applying a query release mechanism with given
privacy and accuracy properties to a confidential database. Formally, in
terms of the differential privacy model summarized in Section \ref%
{subsec:dpandsdl}, the answers to a fixed set of queries with $\left( \alpha ,\beta
\right) $-accuracy from the MWEM query release mechanism with $\left(
\varepsilon ,\delta \right) $-differential privacy are published by the
agency. Any individual may, therefore, use these statistics for any purpose.
Hence, they are public goods because their use is both non-rival and
non-exclusive.

We also assume that the $\varepsilon $ parameter of the $\left( \varepsilon
,\delta \right) $-differential privacy guarantee is a public good. Such an
assumption means that all citizens are protected by the same $\left(
\varepsilon ,\delta \right) $-differential privacy parameters even though
they may place different utility values on $\varepsilon $. This is our
interpretation of the \textquotedblleft equal protection under the
law\textquotedblright\ confidentiality-protection constraint that most
national statistical agencies must provide. See, for example, U.S.\ Code
Title 13 and Title 44 for an explicit statement of this provision for the
American data laws that govern the U.S.\ Census Bureau \citep{title13} and
American statistical agencies in general \citep{cipsea}.

In this equal-protection sense, privacy protection is non-exclusive in
consumption in the same manner as access to legal recourse through the
courts is non-exclusive--it is a right of citizenship. But unlike access to
the courts, where there is rivalry in consumption because one party's
litigation congests the access of an unrelated party's litigation, statutory
privacy protection is non-rival when it is provided via differential
privacy. The reason for the non-rivalry is that the differential privacy
protection is \textquotedblleft worst case\textquotedblright\ protection. If
the query release mechanism's worst possible breach is limited by the
differential privacy bounds, then every citizen's protection is increased or
decreased when the bounds are tightened or loosened, respectively. Alice can
have more privacy in this sense if and only if Bob also enjoys the same
increment. There is no crowding out of one party's privacy protection when
privacy protection is provided to another party.

In our formal setup, only the published-data accuracy parameter $\alpha $
and the privacy protection parameter $\varepsilon $ are considered explicit
objects of production and consumption. These are the formal public goods. We
hold the other parameters of the data publication process constant. It is a subject for future work to make these choices
endogenous.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: abowd-schmutte-privacy
%%% End:


==> deletes.tex <==
%TCIDATA{Version=5.50.0.2960}
%TCIDATA{LaTeXparent=0,0,sw-edit.tex}
                      

% -*- latex -*-
%
% deletes.tex
% Part of abowd-schmutte-privacy.tex

From section: suboptimality, model setup

Ghosh and Roth operate a mechanism that provides a different privacy
guarantee to each record in the database using a model in which privacy
protection is individual-specific, denoted by $\varepsilon _{i}$. See
Appendix \ref{app:GR} for a detailed summary of the Ghosh and Roth proof
that their private auction mechanisms must purchase exactly the same value
of privacy loss, $\varepsilon ^{VCG}$, from each member of the population
who agrees to sell data-use rights and at the same price. This will result
in a query release mechanism in which $k\leq n$ individuals sell data-use
rights, total population privacy loss of $\varepsilon =k\varepsilon ^{VCG}$,
and total payments of $k\gamma _{k+1}$, where $k$ is the index of the
marginal participant when the $\gamma _{i}$ are sorted in increasing order.

At first glance, this is at odds with the notion of privacy protection as a
public good. However, since GR show in their Theorems 3.1 and 3.3 that the
minimum cost mechanism always affords the same level of privacy, $%
\varepsilon ^{VCG}$, to each individual who sells a data-use right, we note
that all members of the population receive $k\varepsilon ^{VCG}$ privacy
protection in aggregate, not just those who sold data-use rights, and even
those members of the population who would have sold substantially more than $%
\varepsilon ^{VCG}$ get $k\varepsilon ^{VCG}$ protection in aggregate. 

Inframarginal individuals, and individuals who do not sell their data-use
rights all receive the same $\varepsilon $-differential privacy protection
because the differential privacy bound on inferential disclosure is
worst-case protection. The Ghosh and Roth analysis therefore illustrates our
key point: $\varepsilon $ is inherently public. Such a property may not hold
for all privacy protection models, but the public-good nature of the
\textquotedblleft worst-case\textquotedblright\ property of differential
privacy protection is directly established by their theorems.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: sw-edit
%%% End:


==> discussion.tex <==
%TCIDATA{Version=5.50.0.2960}
%TCIDATA{LaTeXparent=0,0,sw-edit.tex}

% -*- latex -*-
%
% Time-stamp: <02/03/14 16:29:52 vilhuber>
%              Automatically adjusted if using Xemacs
%              Please adjust manually if using other editors
%
% discussion.tex
% Part of abowd-schmutte-EC2013.tex

The contribution of this paper has been to insert the economic theory of public goods into the discussion of the optimal tradeoff between data privacy and statistical accuracy. The relatively new concept of differential privacy affords a natural interpretation of privacy as a commodity over which individuals might have preferences. In many important contexts, privacy and accuracy are not pure private commodities. If so, the market allocation might not be optimal. Furthermore, it is feasible, at least in principle, to determine the optimal tradeoff between privacy an accuracy.

With these concerns in mind, we have developed a framework for assessing the positive and normative implications this kind of theory. From a positive perspective, we predict that private provision of statistics will be suboptimal, and in particular, will oversupply privacy at the expense of accuracy. From a normative perspective, we provide a rough measure using data from the GSS of the optimal tradeoff between privacy loss and accuracy loss, and calibrate the optimal levels of accuracy and data quality. 


%%% Local Variables:
%%% mode: latex
%%% TeX-master: abowd-schmutte-EC2013
%%% End:

